Maximizing the practical achievability of quantum annealing attacks on factorization-based cryptography

This work focuses on quantum methods for cryptanalysis of schemes based on the integer factorization problem and the discrete logarithm problem. We demonstrate how to practically solve the largest instances of the factorization problem by improving an approach that combines quantum and classical computations, assuming the use of the best publicly available special-class quantum computer: the quantum annealer. We achieve new computational experiment results by solving the largest instance of the factorization problem ever announced as solved using quantum annealing, with a size of 29 bits. The core idea of the improved approach is to leverage known sub-exponential classical method to break the problem down into many smaller computations and perform the most critical ones on a quantum computer. This approach does not reduce the complexity class, but it assesses the pragmatic capabilities of an attacker. It also marks a step forward in the development of hybrid methods, which in practice may surpass classical methods in terms of efficiency sooner than purely quantum computations will.

==> sections/Acknowledgment.tex <==
% ACKNOWLEDGMENT 
% use section* for acknowledgement
\section*{Acknowledgment}

%The authors would like to thank experts for their appropriate and constructive suggestions to improve this template.

==> sections/REFERENCES.tex <==
%REFERENCES
%\section{REFERENCES}
%\balance
%% REFERENCES
%
%\begin{thebibliography}{99}
%	\bibitem{smith2015} J. Smith, "Title of the paper", \emph{Journal name} 12 (3), 45--67 (2015).
%	\bibitem{young2015} M. Young, "The Technical Writer’s Handbook", Mill Valley, Toronto, 2015.
%	\bibitem{apostoli2012} P. Apostoli and A. Kanda, "Cantorian sets, fuzzy sets, rough sets and fregean sets", \emph{Bull. Pol. Ac.: Tech.} 50 (3), 247-276 (2012).
%	\bibitem{nicole} R. Nicole, "Title of paper with only first word capitalized", J. Name Stand. Abbrev., (to be published).
%	\bibitem{blue2007}	A. B. Blue, "Book style with paper title and editor", 	in Title, 1nd ed. vol. 1, C. Editor, Ed. City: Publisher, 2007, pp. 10–50.
%	\bibitem{one2015}	F. One, G. Two, H. Three, and I. Four, "Journal style", Journal, vol. 1, Jan. 1999, pp. 140–151 [Conference, 2015, pp. 300-307].
%	\bibitem{zet2011}	F. Zet and Z. Xix, "Journal style", Journal, vol. 2, pp. 1–21, Jan. 2011.
%	\bibitem{big2009}	J. A. Big, "Periodical style", Periodical, vol. 1, no. 1, pp. 30–38, Jan. 2009.
%	\bibitem{green2014}	K. A. Green, "Published Conference Proceedings style", in Proc. Conference, City, 2014, pp. 18–26.
%	\bibitem{white2013}	L. A. White and M. Black, "Presented Conference Paper style", presented at Meeting (Conference), City, Jan. 2–7, 2013, Paper identifier (optional).
	
%\end{thebibliography}


% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

%\begin{IEEEbiographynophoto}{Jane Doe}
%Biography text here.
%\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}








